A Strategy Language for Controlled Proof Search

This paper introduces the strategy language of Pgeon, a meta-prover with a clear separation between inference rules and proof search. We give the semantics of strategies as functions over proof states, and of the operators that are used to combine them, allowing for sequential composition, choice, repetition and interleaving of strategies. This language is designed to handle the challenge of fair proof search in semi-decidable logics, where simple depth-first exploration of the proof space is not guaranteed to achieve completeness. We showcase the expressiveness and effectiveness of the approach through case studies in first-order and modal logics.

==> eptcsdata.tex <==
\providecommand{\firstpage}{58}
\providecommand{\publicationstatus}{Hermant, Tourret (Eds.): International Workshop on Logical Frameworks\\and Meta-Languages, Theory and Practice (LFMTP 26)\\
EPTCS 448, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.448.5}{10.4204/EPTCS.448.5}}
\pdfoutput=1

